Online Bayesian changepoint detection for network Poisson processes with community structure

Network point processes often exhibit latent structure that govern the behaviour of the sub-processes. It is not always reasonable to assume that this latent structure is static, and detecting when and how this driving structure changes is often of interest. In this paper, we introduce a novel online methodology for detecting changes within the latent structure of a network point process. We focus on block-homogeneous Poisson processes, where latent node memberships determine the rates of the edge processes. We propose a scalable variational procedure which can be applied on large networks in an online fashion via a Bayesian forgetting factor applied to sequential variational approximations to the posterior distribution. The proposed framework is tested on simulated and real-world data, and it rapidly and accurately detects changes to the latent edge process rates, and to the latent node group memberships, both in an online manner. In particular, in an application on the Santander Cycles bike-sharing network in central London, we detect changes within the network related to holiday periods and lockdown restrictions between 2019 and 2020.

==> sections/theory.tex <==
\section{Theoretical justifications for the algorithm}

The work of \cite{wang2019} establishes frequentist consistency and asymptotic normality results for VB methodology. The results of this work rest upon the model satisfying three assumptions, which we give below in Assumptions \ref{ass:VB_one} - \ref{ass:VB_three}. We must verify that each of these results hold for our model, from which the results of \cite{wang2019} will follow.\\

We define what the authors refer to as the \textit{variational log-likelihood}, given as
\[
M_n(\theta;x) := \sup_{q(z)\in\mathcal{F}^n}\int q(z) \log\frac{p(x,z|\theta)}{q(z)} dz
\]

\begin{assumption}[Prior mass]
    \label{ass:VB_one}
    The prior mass with Lebesgue-density $p(\theta)$ on $\Theta$ is continuous and positive on a neighbourhood of $\theta_0$. There exists a constant $M_p > 0$ such that $|(\log p(\theta))''| \leq M_p \exp\left(|\theta|^2\right)$.
\end{assumption}

\begin{assumption}[Consistent testability]
    \label{ass:VB_two}
    For every $\epsilon > 0$ there exists a sequence of tests $\phi_n$ such that
    \[
    \int \phi_n(x)p(x,z|\theta_0) d z d x \to 0
    \]
    and
    \[
    \sup_{\theta:\lVert\theta - \theta_0\rVert \geq \epsilon}\int(1-\phi_n(x))\frac{\ell(\theta;x)}{\ell(\theta_0;x)}p(x,z|\theta_0)d z d x \to 0
    \]
\end{assumption}

\begin{assumption}[Local asymptotic normality (LAN)]
    \label{ass:VB_three}
    For every compact set $K \subset \mathbb{R}^d$, there exist random vectors $\Delta_{n,\theta_0}$ bounded in probability, and nonsingular matrices $V_{\theta_0}$, such that
    \[ 
    \sup_{h\in K}\left|M_n(\theta + \delta_n h; x) - M_n(\theta;x) - h^TV_{\theta_0}\Delta_{n,\theta_0} + \frac{1}{2}h^TV_{\theta_0}h\right| \overset{P_{\theta_0}}{\rightarrow} 0 
    \]
\end{assumption}

To satisfy Assumption \ref{ass:VB_two}, it suffices that there exist a consistent estimator $T_n$ of $\theta$, as one can simply set $\phi_n := \mathbb{I}\{T_n - \theta \geq \epsilon/2\}$ \citep{wang2019}. Assumption \ref{ass:VB_three} is the most technically demanding and will require model-specific analysis. 

\begin{proof}
    Consider a Taylor expansion of the log-likelihood $\ell(\theta;x,z)$ about the true parameter value $\theta^* = (\pi^*, \mathrm{vec}(\lambda^*)) := (\pi^*, \lambda_v^*)$:
    \begin{align*}
    \ell(\pi^* + \delta_n^\pi h^\pi, \lambda_v^* + \delta_n^{\lambda_v} h^{\lambda_v}) &= \ell(\pi^*, \lambda_v^*) + (h^\pi)^T\delta_n^\pi \nabla_\pi \ell(\pi^*,\lambda_v^*) + (h^{\lambda_v})^T\delta_n^{\lambda_v} \nabla_{\lambda_v} \ell(\pi^*,\lambda_v^*) \\
    &+ \frac{1}{2}\left((h^\pi)^T\delta_n^\pi H_\pi (\pi^*,\lambda_v^*)\delta_n^\pi h^\pi + (h^{\lambda_v})^T\delta_n^{\lambda_v}H_{\lambda_v}(\pi^*,\lambda_v^*)\delta_n^{\lambda_v}h^{\lambda_v}\right) + o_P(1)
    \end{align*}
    Our complete likelihood takes the form
    \[
    \log p(x,z|\pi, \lambda) = \sum_i \sum_k \tilde z_{ik}\log \pi_k + \sum_{i\neq j}\sum_{k,m}\tilde z_{ik}\tilde z_{jm}\left(x_{ij}\lambda_{km} - T\lambda_{km}\right)
    \]
    subject to the constraint that $\sum_k \pi_k = 1$. 
\end{proof}

